Mathematical modeling of cholera epidemics in South Sudan

In this work, we analyze and model the cholera epidemics that affected South Sudan, the newest country in the world, during 2014 and 2015. South Sudan possibly represents one of the most difficult context in which adapt the deterministic mathematical cholera model, due to the unstable social and political situation that clearly affects the fluxes of people and the sanitary conditions, increasing the risk of large outbreaks. Despite the limitation of a static gravity model in describing the chaotic human mobility of South Sudan, the SIRB model, calibrated with a data assimilation technique (Ensemble Kalman Filter), retrieves the epidemic dynamics in the counties with the largest number of infected cases, showing the potentiality of the methodology in forecasting future outbreaks.

==> codes/centroid.tex <==
\begin{lstlisting}[frame=trBL][caption={Pseudo - code for centroid calculations},label=codedistance]
% Input file: population distribution and payam division raster images
[population] = geotiffread (population raster image);
[payams] = geotiffread (payam raster image);
.
. %adjusting the format of the matrices.
.
% Identification of the payam through the ID number
ID = unique (payams);
% Check the number of payam
if length(ID) != 263
	display ('Error')
end
% Defining the grid to scan the raster
low longitude limit= 29;
high longitude limit = 36;
low latitude limit = 3;
high latitude limit = 12;
cell size = 0.0033332;

Xgrid = low longitude limit:cell size:high longitude limit;
Ygrid = low latitude limit:cell size:high latitude limit;
grid = meshgrid [Xgrid, Ygrid];

% storing positions of the centers of the cells with population values;
position pop = population.*grid;

% Pre - allocation of the variable that will contain the coordinates as longitude and latitude
centr = zeros(length (ID), 2);     

% Compute the centroid using MATLAB toolbox GEOM2D
for i := 1 to ID
	% calculating the population in the area
	total pop (i) = sum(population(payams = ID(i)));
    . 
    .
    % compute the centroid
    .
    .
    centr(i) = position pop(population(payams = ID(i)))/total pop(i); 
    .
    % Check whether the point is inside the area
    if payam(centr(i)) ! = ID(i)
    	.
    	% Use a function in the toolbox GEOM2D that constrict the centroid to change it's position
        centr(i) = cons_centroid(centr(i));
    end
end
\end{lstlisting}

==> codes/distance.tex <==
\begin{lstlisting}[frame=trBL][caption={Pseudo - code for distances calculations},label=codedistance][firstnumber=1]
% Transform coordinates in radians to apply the haversine formula
lat = lat.*2*pi/360;
long = long.*2*pi/360;

R = 6371; 							 % Earth radius in km 

% Pre - allocation of the variable d, defining a matrix in which we store the reciprocal 
% distances between points. The size is 263 x 263 
d=zeros(size(long),size(lat));       % distances
% Compute the distance and fill the matrix
for i:= 1 to size(d,1)
	for j:= 1 to size(d,2)
    	.
        .
        d = 2R * arctg2 (sqrt(a),sqrt(1-a));
    end
end
\end{lstlisting}

==> codes/raincentr.tex <==
\begin{lstlisting}[frame=trBL][caption={Pseudo - code to read rainfall data},label=coderainarea][firstnumber=last]
% from the vector of the centroid we define longitude and latitude
long = centr(:,1);
lat = centr(:,2);
% Interpolation of the daily rainfall data in the centroids
for i:= 1 to date 			%daily values
	rain in centroid(:,j) = interp2 (X,Y,rain(j),centr(1),centr(2));
end

% Input file: rain matrices and payam division raster image
[payams]= geotiffread(payam raster image);
.
. %adjusting the format of the matrices.
.
% Pre allocating the variable in which store a daily rain value for each payam
rain value = zeros(ID, date);

for j:= 1 to length(date)
	for i:= 1 to length(ID)
    	rain value = mean(rain(payams==ID(i)));
        if payams != ID(i)
        	rain value (i,j) = rain in centroid (i,j);
        end
    end
end
\end{lstlisting}

==> codes/rainmap.tex <==
\begin{lstlisting}[frame=trBL][caption={Pseudo - code to read rainfall data},label=coderainmap][firstnumber=last]
% scan the precipitation tensor in the period of analysis
for k := 1 to length(date)
	% define a figure environment
	figure
    .
    .
    % function to plot the rain date in day k
    mapshow(X,Y, rain(k))
    .
    % function to overlap the map of the model domain
    hold on
    % read the map in shapefile format
	shapefile=shaperead(model domain shapefile);
    % function to plot the map
    mapshow(shapefile);
end    
\end{lstlisting}

==> codes/rainurl.tex <==
\begin{lstlisting}[frame=trBL][caption={Pseudo - code to read rainfall data},label=coderainurl][firstnumber=1]
% Connecting the code to the database:
url = 'iridl.ldeo.columbia.edu';
%read the time vector T, and the coordinates X and Y
date = ncread (url,'T');
X = ncread (url,'X');
Y = ncread (url,'Y');
% Read the value of the precipitation in the tables
% We define a tensor that contains for each day in T the grid containing rainfall data
rain = double(ncread (url, 'precipitation'));
\end{lstlisting}

==> greetings.tex <==
\newpage
\thispagestyle{empty}
This page is intentionally left blank.
\newpage
\chapter*{Acknowledgment}
%\addcontentsline{toc}{chapter}{Acknowledgment}
\thispagestyle{empty}
I have started working on this thesis with enthusiasm from the very first day. It would not be so if not for the passion and the enthusiasm that all the team of the ECHO-Lab at the EPFL showed through their words. I immensely thank Professor Andrea Rinaldo, for welcoming me in the Lab and for giving me this opportunity.  I am immensely thankful as well to my supervisors, Enrico Bertuzzo, Flavio Finger and above all Damiano Pasetto, for the support and the patience, for your willingness, your helpfulness and your precious teachings. I have learned a lot from you and the Lab all, and definitely, this was a really good and inspiring experience. Thanks to Andrew Azman, for your precious advice and your suggestions.
\\ \par Gratitude deserve as well all the people that, here and around the globe, shared with me this experience. 

Thanks to old and new friends that I met during this strange year passed in Lausanne. One way or another, you all gave me emotions, sharing laughs, nerves or beers. I am sure I will see you again, somewhere.

Thanks overall to my girl friends Roberta, Maria and Meritxell, for the daily dose of 'flower-power', for being my Italian-Spanish family in Switzerland. Remember, we have an agreement.

Thanks to the people that were with me with their thoughts.

To Walter, for your brotherhood and your constant faith in me.

To Chiara, for your almost-daily long-distance calls and your advices.

To Ilaria, Martina and Emanuela, for our "strong-no-matter-distance" friendship.

To my physicists, especially Francesco, for the mathematical support in writing down this report and to have opened my mind to research.

To all the friends in Turin that made me feel their love.
\\ \par Last, but of course not least, thanks to my family that gave me the possibility of an education, to study and to be here, and that made me the person I am today: to my Mother, the reason why I have reached so much in life; to my Father, whose teachings and experiences always moved me to think. To my sister Rita, for inspiring me everyday since I was a child. To my sister Amalia, from whom I have learned the joy to follow instincts. To my brother Rafael, whose strength to me is an example. 
\\ \par In ultimo, ma non per importanza, vorrei ringraziare la mia famiglia che mi ha dato la possibilità di un'educazione, di studiare e di essere qui, e che mi ha resa la persona che sono oggi: a mia Madre, il motivo per il quale ho raggiunto così tanto nella vita; a mio Padre, i cui insegnamenti ed esperienze mi hanno sempre spinta a riflettere. A mia sorella Rita, per inspirarmi ogni giorno da quando ero una bambina. A mia sorella Amalia, dalla quale ho imparato la gioia di seguire gli istinti. A mio fratello Rafael, la cui forza è per me un esempio.

\begin{center}
\emph{"If you'll believe in me I'll still believe!"}
\end{center}





==> pretext.tex <==
\newpage
\thispagestyle{empty}
\setcounter{page}{2}
~\vspace*{600pt}
\begin{flushleft}
All the maps in this work were processed with the use of ArcGIS 10.3 from data and shapefiles made available from the South Sudan Government, the South Sudan National Bureau of Statistics and the World Health Organization. 
In order to maintain the authenticity of these information, we tried to minimize the number of modifications to the least possible yet adequate to allow us to analyze the new acquired information. Misfitting between shapefiles and different spelling of toponyms are possible. 
\end{flushleft}
